DiffuseLoco: Real-Time Legged Locomotion Control with Diffusion from Offline Datasets

This work introduces DiffuseLoco, a framework for training multi-skill diffusion-based policies for dynamic legged locomotion from offline datasets, enabling real-time control of diverse skills on robots in the real world. Offline learning at scale has led to breakthroughs in computer vision, natural language processing, and robotic manipulation domains. However, scaling up learning for legged robot locomotion, especially with multiple skills in a single policy, presents significant challenges for prior online reinforcement learning methods. To address this challenge, we propose a novel, scalable framework that leverages diffusion models to directly learn from offline multimodal datasets with a diverse set of locomotion skills. With design choices tailored for real-time control in dynamical systems, including receding horizon control and delayed inputs, DiffuseLoco is capable of reproducing multimodality in performing various locomotion skills, zero-shot transfer to real quadrupedal robots, and it can be deployed on edge computing devices. Furthermore, DiffuseLoco demonstrates free transitions between skills and robustness against environmental variations. Through extensive benchmarking in real-world experiments, DiffuseLoco exhibits better stability and velocity tracking performance compared to prior reinforcement learning and non-diffusion-based behavior cloning baselines. The design choices are validated via comprehensive ablation studies. This work opens new possibilities for scaling up learning-based legged locomotion controllers through the scaling of large, expressive models and diverse offline datasets.

==> sections/unsed_text.tex <==
% % 回答三个问题
% % What is the problem
% % Why is this prob hard
% % How to solve the prob

% % Contribution
% % 1. Open a new possibility for learning legged locomotion control from offline datasets
% % 2. Multiskill control with one policy without latent variable conditioning
% % 3. Goal conditioning
% % 4. Diffusion realtime control
% % 5. Deployment choice leads to real-time control → leads to onboard compute control (机器人背着走)


% % Multi-skill RL not learning well, especially without conditioning 
% % 

% % \begin{figure*}
% %     \centering
% %     \includegraphics[width=0.999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999999\textwidth]{figures/cassie-and-go.png} %?????
% %     \caption{Snapshot showing the Cassie and Go1 robot walking with our policy. Go1 (top) is running onboard computing for our diffusion model. Cassie (bottom) is running in simulink? with our diffusion model.}
% %     \label{fig:cassie-and-go}
% % \end{figure*}

% % Developing controllers for high-dimensional continuous
% % control systems such as legged robots has long been an
% % area of study. The landscape of legged robotics control has primarily been dominated by model-based and learning-based strategies. However, these methods often encounter limitations Early work in this field focused on developing
% % approximate dynamics models of a system and then using trajectory optimization algorithms to solve for the actions that lead an agent to achieve a desired goal [1]–[4]. However, the resulting controllers tend to be highly specialized for a particular task, limiting their ability to generalize across more diverse tasks or environments. More recently, there has been a surge in algorithms that use reinforcement learning (RL) to learn locomotion behaviors [5]–[9]. However, the challenge remains when considering the necessity of multitask learning, a feat that existing RL policies struggle to achieve efficiently. This gap in capability underscores the need for a more versatile and robust control strategy.

% % Enter the realm of diffusion models in robotics. Recent advancements in this area have shown promising results in visuomotor policies and motion prediction, particularly in stable, static-base systems. However, the application of these models to more dynamic systems, like legged robots, has remained largely unexplored due to their inherent instability and computational demands.

% % In this work, we propose DiffuseLoco, a novel framework that leverages the strengths of diffusion-based policies and learning from offline datasets, addressing critical limitations in existing methodologies. By integrating the power of diffusion models with a comprehensive offline dataset, our framework sets a new standard in learning multi-modal locomotion skills. This approach not only overcomes the limitations of traditional RL methods, particularly in the context of exploration difficulties and data utilization, but also demonstrates a remarkable capacity for real-time control in dynamic environments.

% % Our contributions are multifaceted. 

% % \begin{enumerate}
% %     \item This work introduces the first methodology capable of achieving stable multi-skill control using a single policy framework. Notably, this method does not rely on latent variable conditioning and can be applied in a zero-shot transfer manner. 
% %     \item A novel architectural approach is presented, distinguishing between goal-conditioning and state-conditioning. This distinction proves particularly beneficial for systems with diverse and rapidly changing states, offering better performance to handle tasks that require a high degree of responsiveness and adaptability.
% %     \item Innovative modifications to enhance real-time applicability of diffusion models in dynamic environments like quadrupedal robots. This includes the integration of delay observation and other design choices, addressing the challenge of deploying complex models in real-time scenarios. 
% %     \item This work demonstrates the possibility for learning legged locomotion control from offline datasets, which stands for a more efficient and scalable method in teaching complex locomotion skills to robots.
% % \end{enumerate}

% % We present a unique methodology enabling stable multi-skill control using a single policy framework, a novel architectural distinction between goal-conditioning and state-conditioning, and innovative modifications enhancing the real-time application of diffusion models. These advancements collectively pave the way for more efficient, scalable, and robust control strategies in teaching complex locomotion skills to robots.


% % \zli{Data driven learning}
% % We have witness IL from offline dataset, scale up leads to generalization, scale up from 2 perspectives: data, architecture. IL is promisng route, espeicaly in robotics. have been applied xxxxxx, but, manipulation tasks in robotics, ee traj, low replan frequency, inherently more stable dynamics (static-based arm, etc). However, questions has arised, how can we harness the capacity if IL to the tasks that require real-time control that requires higher frequency and on a more dynamic system, such as legged robots. 



% % Mutli-modal xxx
% % Leverage offline dataset

% % Short intro to legged robots.
% % \zli{legged robotics community has realized the advantages of building controller from data. In the recent years, online RL enables the legged robots to acquire dynamic locomotion skills with considerable robutness in the real world. Howerever, say some challenging, such as multitask RL}


% % \zli{Reward engineering in RL versus dataset engineering in IL. this could be controversal. focus more on multi-modal distribution}
% % , where its tends to overfit to a single skill and diminishes diverse environments.


% % Due to the deficiency of multimodal expressiveness within the Proximal Policy Optimization (PPO) algorithm \cite{schulman2017proximal}, 

% % Additionally, the data requirement in online RL is substantial. Basic walking policies necessitate over 100 million transitions \cite{Peng2020Learning, Shao2022Learning}, while multi-skill algorithms like Adaptive Motion Planning (AMP) may require up to 4 billion environment steps \cite{9981973}. Furthermore, each new skill integrated within the same policy framework demands a similar voluminous data process. 
% % \zli{I doubt this is the drawback of online RL -- without RL-based policy providing good data, IL can not learn. Also, IL needs more data than RL (which learns from scratch).}



% % On the other hand, models with a smaller number of parameters may fail to capture the diversity and multi-modality inside the dataset, limiting its applicability. 


% In real-world benchmarks on quadrupeds locomotion task, \method achieves better performance compared to existing multi-skill RL policies and Behavior Cloning (BC) baselines, achieving higher success rate, stability and lower velocity tracking errors. More importantly, our policy is able to walk steadily with several distinct gaits, pacing and trotting, under exactly the same commands, demonstrating its ability to learn multi-modality in the dataset.
% Furthermore, we demonstrate the ability to locomote on easy terrains and various ground friction


% % Move this to later sections
% % Furthermore, creating a smooth action trajectory while accounting for the distribution shift and possible dataset overfitting also sets difficult challenges for locomotion feedback control.


% % \zli{this paragrah is good, but I wonder if we can also mention the *feedback control* instead of just real-time which sounds more like engineering efforts (to accelerate the large model). Talking about the large model, you can also metion that, the drawback of the IL is that, it needs to scale up, by using large model, which could be slow during inference. Then, the drawback leads to the limits of controls, then what we aim to solve in this paper.}


% % Data-driven learning with offline data at scale has witnessed exciting progress in many fields, including computer vision and natural language processing, where the scaling up of both model size and data size leads to better generalization ability and better capacity. \cite{Kaplan2020Scaling, Sun2017Revisiting}. 
% % In robotics, imitation learning (IL) from offline datasets has also been demonstrated as a promising route that leads to more scalable policies and has been applied in fields including manipulation \cite{brohan2023rt2, brohan2023rt1} and autonomous driving \cite{chen2019deep, codevilla2018end, pan2017agile}. 
% % However, these applications only reflect a subset of robotics that involves a low-dimensional action space (\textit{e.g.}, end-effector trajectory) with low-replanning frequency on inherently stable systems. 
% % An interesting question arises: how can we harness the capacity and advantages of IL from diverse offline datasets for the domain of realtime feedback control on more dynamic systems, such as legged robots? 


% % \zli{Overall comments of this section: the intro can be cut further. intro should be concise and high-level description. you can move the details of pros and cons of sepcfic methods into literature review. moreover, the contributions read quite detailed. will be better to provide a broader view instead specific points. or you can group all specici metric into one point.}

% % There are apporach that utilize data to develop controller, i.e.,data-driven control, such as adaptive control~\cite{adaptctl}, learning mpc~\cite{learningmpc}, or gaussain process~\cite{gaussprocess}, most of them deal with simple system or only a small part utlize data. 
% % Recently, we observe trend using deep model-free RL to develop controller for dynamic systems, such as from robot arm~\cite{armrl}, to quadrotors~\cite{quadrl}, to legged robots~\cite{legrl}. This results in a more end-to-end method, from observation directly to joint-level command. 
% % say some advantages.
% % However,


% Learning with offline data at scale has witnessed exciting progress in many fields, including computer vision and natural language processing. 

% In robotics, imitation learning (IL) from offline datasets has also been demonstrated as a promising route that leads to more scalable policies and has been applied in fields including manipulation \cite{brohan2023rt2, brohan2023rt1} and autonomous driving \cite{chen2019deep, codevilla2018end, pan2017agile}. 


% \zli{Supervised} learning with offline data at scale has been shown promising in the deep learning fields, such as computer vision and natural language processing. \zli{cite\cite{}}
% In robotics, imitation learning (IL) from offline datasets has also been demonstrated as effective in developing more scalable policies and has been applied in fields including robotic manipulation \cite{brohan2023rt2, brohan2023rt1} and autonomous driving \cite{chen2019deep, codevilla2018end, pan2017agile}. 
% However, these applications only reflect a subset of robotics that involves a low-dimensional action space (\textit{e.g.}, end-effector trajectory) with low re-planning frequency on inherently stable systems (\textit{e.g.}, robot arms or cars). 
% Training policies from offline datasets and applying zero-shot transfer on legged robots for real-time feedback control have largely remained an underexplored topic. 

% Large models, especially diffusion models, are powerful generative models commonly used in computer vision and image generation~\cite{ryu2022pyramidal, rombach2022highresolution}. 
% % scaling up of both model size and data size leads to better generalization ability and better capacity. \cite{Kaplan2020Scaling, Sun2017Revisiting}
% However, unlike the success achieved in those areas, these models cannot be deployed online for feedback control, and deploying onboard for edge computing is at a higher level of difficulty. 

% An interesting question arises: how can we harness the capacity and advantages of large-scale models learning from diverse offline datasets for the domain of real-time feedback control on more dynamic systems, such as legged robots? 


% However, unlike the success achieved in those areas, these models cannot be deployed online for feedback control, and deploying onboard for edge computing is at a higher level of difficulty. 


% Training policies from offline datasets and applying on more dynamic robots for real-time feedback control is still an underexplored topic. 


% \zli{put this to somewhere later}
% Furthermore, unlike online RL, learning from offline data means we could keep growing the dataset and absorb diverse skills without recollecting data from pre-trained policies. 


% On the contrary, there have not been prior attempts to leverage diffusion models to learn real-time control on complex dynamic systems, 


% Leveraging a diffusion-based approach, \method demonstrates proficiency in learning multiple locomotion skills from a diverse range of offline datasets and be deployed for feed-back control onboard. \tkk{Illustrated in Figure \ref{fig:workflow-diagram} and detailed in Algorithm \ref{algo:workflow}, our framework is composed of three stages, with an emphasis on quadrupedal locomotion control to exemplify its application. It is important, though, to highlight that \method's design ensures its applicability to a broad spectrum of control tasks beyond the example provided.}



% % % \begin{remark}
% % % data can come from any locomotion control policies, not limited to RL policies, but are more MPC etc. but, current limit of using MPC as dataset -- talk about why we cannot use MPC in this work (frequency)
% % % \end{remark}

% % \begin{remark}
% % Current limit of using Model-Predictive-Control (MPC) as dataset mainly includes difference in frequency: MPC does not work out-of-the-box at a lower frequency of 30Hz as RL policy runs at. 
% % \end{remark}

% % state challenge of diffusion as control

% %%ZL:01/28: the section looks more interesting than the previous one, it will be better to make it appear earlier.
% %%ZL:01/28: better folow could be, starting with this general and versatitle framework, and explain the architecture, and diffusion. then dataset, then real-time deployment. 

% % In order to learn the dataset that features multi-modality, we propose \emph{\method}, a diffusion-based policy for learning multi-skill locomotion tasks that require real-time control on highly dynamical systems. In \Cref{sec:method-arch}, we describe the components of \method, which include a DDPM for predicting actions and conditioned on directly on proprioceptive observations and velocity commands. Next, in \Cref{sec:method-training}, we detail how we train \method in an end-to-end fashion from offline locomotion demonstrations.

% % The following paragraphs provide a comprehensive explanation of the development of this model, including its structure, training process, and design choices for real-time control.



% % \subsection{Architecture for Real-Time Control}
% % \label{sec:architecture-for-realtime-control}
% % 1. Architecture and goal conditioning
% % 2. Deployment Choices
% % diffusion is slow, so, in this section, we focus on tackling real-time control leveraging diffusion policy


% % Furthermore, creating a smooth action trajectory while accounting for the distribution shift and possible dataset overfitting also sets difficult challenges for locomotion feedback control.


% % 1. Limited attempts in learning locomotion tasks directly from offline datasets. 
% % 2. Existing easier tasks in simulation env, such as Gym locomotion tasks. 
% % 3. Methods: mainly Offline RL: Cal-QL, CQL, IQL DT
% % Not been demonstrated in real-world
% % 4. Some prior works learn offline as bootstrapping for online learning. 
% % 5. Others seek transfer learning from offline datasets. 

% % While there is a breadth of work in initializing agents with
% % prior data to bootstrap from [75–80],

% % \cite{smith2023learning} Transfer learning

% % \zli{prediction to mitigate delaly in real time control}
% % Learning from offline dataset has drawn heats in robotics tasks, such as manipulation and mobile manipulation \cite{}. 



% %%ZL:01/28: this section reads quite important to the method, will be better to have a figure to visualize it. 
% % \zli{Starting with the main point, then talk about reasoning and details}

% % \zli{Mention that diffusion model has the capacity to learn such a delay. refer to RL does not have this capacity, usually less than one control step. Table IV, \cite[Table IV]{zli}}
% % A \zli{(another)} critical aspect of meeting real-time requirements in our system is optimizing the control flow of our policy. Central to this optimization is the challenge of generating accurate and timely motions. Ideally, the policy should use the most recent observational inputs to produce the most effective motions. However, the time required to perform the inference typically exceeds the constraints of real-time processing. \zli{for example, xx sec}

% % To address this, we find that the capacity of \method is enough to predict actions with one-step delayed observation. 



% % This approach allows us to maintain a balance between real-time responsiveness and the accuracy of motion generation, ultimately leading to enhanced system performance in dynamic environments.
% % \zli{Larger model may require more time for inference, then this method can be extended by delayed more steps. But a note is that more delayed steps will result in more challenging learning complexity, future work can be solving this by prediction with a speperated policy, etc.}

% % This approach ensures that inference is continuously operating in parallel with motion execution. Consequently, while the system is executing a set of movements, it is simultaneously preparing the next set based on the latest available observations.
% % By employing this strategy, we leverage the high-speed capabilities of our real-time compute pipeline to perform inference at every time step. The key to maximizing performance quality lies in the parallel execution of motion and inference, coupled with the use of only a subset of the generated motions. 

% % \subsection{Receding Horizon Control for Action Sequence Prediction}
% % Similar to \cite{}, we find that receding horizon control helps maintain consistency and smoothness , where at each timestep $t$, $n_p$ timesteps of future actions are predicted, and only the first $n_a$ actions are applied to the system. 
% % \zli{????}


% A possible future work to solve this is to have alternative policies feeding "half-way" diffused outputs to each other, reducing the delay required to run the model. 


% % \zli{The diffusion model is known as being slow as inference, usually can only update at xxx hz. in order to deploy online, people do xxx. An example can be seen at xxxx where training step is while inference step is xxx. However, we find that xxxx is not applicable in more complex control secnarios, such as xxx. Therefore, we propose to use xxxx. In this xxx, xxxxx.}

% The diffusion models are known as being slow for inference, as it requires sequential denoising steps and cannot be parallelized. 


% This is ultimately proved to be detrimental to the robustness of the \method policy. 

%An example can be seen at xxxx where training step is while inference step is xxx. However, we find that xxxx is not applicable in more complex control secnarios, such as xxx. Therefore, we propose to use xxxx. In this xxx, xxxxx.


We train our source locomotion policies of different skills using AMP to prevent extended reward engineering for each skill. When training each skill, we feed the discriminator with only one reference motion from motion capture data \cite{Peng2020Learning} of a real dog, along with appropriate commands for that skill. We acquire four source policies of pacing, trotting, left turning, and right turning, and we distribute the four skills evenly in our dataset. 
For more details on Source Policy training, we refer readers to previous work on AMP~\cite{9981973}. 

% It is primarily due to the exploration problem compared to simpler, single-modal settings in RL~\cite{chua2018deep, pathak2019self}. 
% This problem becomes more pronounced in learning legged locomotion, where a variety of different \textit{skills} can be used to accomplish the same \textit{goal}. 
% We often observe such behavior in the animal kingdom. 
% For example, a dog can use either trotting or pacing \textit{skills}, which have different ground contact sequences, to achieve the same speed.

% Learning legged locomotion controllers modeled by diffusion models can be viewed as a combination of two domains of robotics research: learning-based locomotion control and diffusion models applied in robotics. 

% 1. rl not work multi-task multi-skill

% 2. existing works mostly multi-task single-skill

% 3. some works multi-skill via distillation

% 4. AMP


% One action step
% ours: IL, diffusion, tf, multi-step obs, rhc
% amp: RL, mlp, one-step obs, one-step output, emeshize RL one-time step output
% amp w/ hist: 
% \dt: bc tf, one-step output
% TF-RHC, RHC


% and difficulty in exploration for multimodal reward distribution for off-policy algorithms~\cite{haarnoja2018soft}. 

% However, learning a multi-skill policy with online RL is still a challenge, due to limited multimodal expressiveness for commonly-used Policy Gradient (PG) methods~\cite{tessler2019distributional}


% also achieve better sim-to-real transfer performance on locomotion tasks.


% This leads to smoother trajectory in all five commands, as shown in figure \ref{}, where the magnitude of angular velocities in roll and pitch directions experienced by the robot is reduced from xxx to xxx, a xx times decrement. 

% \subsection{Summary of Results}
% il > bc, tf > mlp, rhc>onestep

% In this research, we have demonstrated that legged robots can be trained to navigate diverse real-world terrains, including floors, mattresses, and grass, using solely offline datasets. This achievement has been made possible through the implementation of the diffusion-based locomotion policy combined with deployment optimizations, such as hardware acceleration and incorporating delayed observations. Through comparisons with various existing baselines, our diffusion-based control method has not only proven to outperform others in terms of efficacy but also exhibited a  capacity for multi-modal expression. The empirical results distinctly highlight that our diffusion-based locomotion control approach is more robust and versatile compared to traditional behavior cloning techniques. This paves the way for a more reliable transition from simulation to real-world applications. Moving forward, we aim to refine and enhance our methodology by integrating larger models and a broader spectrum of training data, further elevating the precision and adaptivity of robot performance in real-world scenarios.



% For future research, we recommend investigating the integration of complex weighted loss functions to recognize and rebalance data, potentially mitigating dataset biases. This approach could enhance the efficiency and fairness of the learning process. Moreover, another promising direction is the development of a unified, large model for legged robot control by integrating a large set of offline data from diverse control sources. This integration could significantly advance the field, drawing parallels with advancements in other learning fields.


% We then demonstrate the different skills learnt by \method can be performed efficiently on hardware. Finally, we test the robustness of \method by introducing different friction and small terrain to the test environment, followed by ablation studies on the design choices we made in Isaac Gym simulation. 



% , and our experiments show that \method trained on our locomotion dataset transfers zero-shot on hardware, exhibits better stability and velocity tracking error compared to all baselines, and can be run onboard the quadrupedal robot. 
